Tyche: Risk-Based Permissions for Smart Home Platforms

Emerging smart home platforms, which interface with a variety of physical devices and support third-party application development, currently use permission models inspired by smartphone operating systems-they group functionally similar device operations into separate units, and require users to grant apps access to devices at that granularity. Unfortunately, this leads to two issues: (1) apps that do not require access to all of the granted device operations have overprivileged access to them, (2) apps might pose a higher risk to users than needed because physical device operations are fundamentally risk-asymmetric-"door.unlock" provides access to burglars, and "door.lock" can potentially lead to getting locked out. Overprivileged apps with access to mixed-risk operations only increase the potential for damage. We present Tyche, a system that leverages the risk-asymmetry in physical device operations to limit the risk that apps pose to smart home users, without increasing the user's decision overhead. Tyche introduces the notion of risk-based permissions. When using risk-based permissions, device operations are grouped into units of similar risk, and users grant apps access to devices at that risk-based granularity. Starting from a set of permissions derived from the popular Samsung SmartThings platform, we conduct a user study involving domain-experts and Mechanical Turk users to compute a relative ranking of risks associated with device operations. We find that user assessment of risk closely matches that of domain experts. Using this ranking, we define risk-based groupings of device operations, and apply it to existing SmartThings apps, showing that risk-based permissions indeed limit risk if apps are malicious or exploitable.

==> Risk-based_ SECDEV_18/stats.tex <==
\newcommand{\participantCount}{400\xspace}
\newcommand{\totalFunctions}{146\xspace}
\newcommand{\expertLow}{62\xspace}
\newcommand{\expertMid}{58\xspace}
\newcommand{\expertHigh}{26\xspace}
\newcommand{\informedLow}{20\xspace}
\newcommand{\informedMid}{57\xspace}
\newcommand{\informedHigh}{69\xspace}
\newcommand{\uninformedLow}{19\xspace}
\newcommand{\uninformedMid}{45\xspace}
\newcommand{\uninformedHigh}{82\xspace}
\newcommand{\informedParticipantCount}{200\xspace}
\newcommand{\uninformedParticipantCount}{200\xspace}
\newcommand{\informedResultperFunction}{100\xspace}
\newcommand{\uninformedResultperFunction}{100\xspace}
\newcommand{\uninformedFailedPearson}{40\xspace}
\newcommand{\informedFailedPearson}{41\xspace}
\newcommand{\uninformedCleanCount}{116\xspace}
\newcommand{\informedCleanCount}{94\xspace}
\newcommand{\totalDeviceTypes}{61\xspace}
\newcommand{\percentDecHighRisk}{60\%\xspace}

